FPGA-based Distributed Union-Find Decoder for Surface Codes

A fault-tolerant quantum computer must decode and correct errors faster than they appear to prevent exponential slowdown due to error correction. The Union-Find (UF) decoder is promising with an average time complexity slightly higher than $O(d^3)$. We report a distributed version of the UF decoder that exploits parallel computing resources for further speedup. Using an FPGA-based implementation, we empirically show that this distributed UF decoder has a sublinear average time complexity with regard to $d$, given $O(d^3)$ parallel computing resources. The decoding time per measurement round decreases as $d$ increases, the first time for a quantum error decoder. The implementation employs a scalable architecture called Helios that organizes parallel computing resources into a hybrid tree-grid structure. Using a Xilinx VCU129 FPGA, we successfully implement $d$ up to 21 with an average decoding time of 11.5 ns per measurement round under 0.1\% phenomenological noise, and 23.7 ns for $d=17$ under equivalent circuit-level noise. This performance is significantly faster than any existing decoder implementation. Furthermore, we show that Helios can optimize for resource efficiency by decoding $d=51$ on a Xilinx VCU129 FPGA with an average latency of 544ns per measurement round.

==> app_decoding.tex <==
\section{Decoding Graph}
\label{sec:decodinggraph}

For clarity, we will only use X errors below as Z errors can be independently dealt with in the same way.

The surface code can be conveniently represented by a graph ${G}({V}, {E})$
 in which vertices represent the ancillas and edges the data qubits. The weight of edge is determined by the probability of error in the corresponding data qubits. This graph is called the \emph{model graph}, which can be constructed off-line by characterizing the error probability of every data qubit
 For distance d surface code, there are $d\times (d-1)$ vertices.
\autoref{fig:model_graph} shows a model graph for $d=3$ surface code.

This model graph can be extended to three dimensional 
in which multiple identical planar layers are stacked on each other. Each layer represents a round of measurement. The total number of rounds is usually the same as the distance of the surface code. 
Corresponding vertices in adjacent layers are connected by edges which represent the probability of measurement error of the corresponding ancilla. 
That is, there are $d\times d\times (d-1)$ vertices in this three-dimensional model graph.

In each round of measurement, some ancillas may report nontrivial outcomes, indicating errors may happen in some data or ancilla qubits. The set of ancillas (and the corresponding vertices in the model graph) of nontrivial measurement outcome is the \emph{syndrome}. The syndrome and the model graph constitutes the basis for decoding algorithms.

The \emph{decoding graph} compactly represents this basis: it is simply the model graph with vertices in the syndrome marked. \autoref{fig:decoding_graph} shows a decoding graph for $d=3$ surface code.

\begin{figure} [!ht]
    % \renewcommand*\thesubfigure{(\alph{subfigure})}  % add parentheses manually
	\centering
% 	\includegraphics[width=0.75\linewidth]{figures/CSS_33.pdf}
	\begin{subfigure}{.47\linewidth}
	    \centering
        \includegraphics[width=1\linewidth]{figures/model_graph.pdf}
        \caption{}
        \label{fig:model_graph}
    \end{subfigure}
    \hfill
	\begin{subfigure}{.47\linewidth}
	    \centering
        \includegraphics[width=\linewidth]{figures/decoding_graph.pdf}
        \caption{}
        \label{fig:decoding_graph}
    \end{subfigure}
    \hfill
	\caption{Model graph and decoding graph of Z-ancillas for d =3 surface code (a) decoding graph consists of all Z-ancilla measurements across multiple rounds as vertices and all possible single qubit errors resulting in changing Z-ancilla measurements as edges (b) decoding graph is model graph with measurement for each vertex added. In this figure trivial measurement results are shown in red.}
	\label{fig:model_n_decoding_graph}
\end{figure}

\begin{comment}
\subsection{Decoding Algorithms}
A decoding algorithm is necessary to identify the underlying error pattern from the decoding graph. 
The output of the decoder will be a probabilistic guess of the underlying error pattern, which will be used to generate a correction pattern. The objective is that when the correction pattern is applied, the chance of the surface code entering a different logical state will be minimized. 

Rate of decoding must be higher than rate of syndrome generation to avoid an exponential slowdown of a quantum computer due to decoding~\cite{Holmes2020Nisq}.
This is caused by T-gates in the quantum circuit, which require the state of the quantum circuit before executing the gate.
At every T-gate the circuit must be paused until error correction up to that state is completed, which causes more syndrome data to keep on accumulating, during the correction.
If the decoder is slower than the rate of syndrome generation, this results in an exponential backlog of syndrome data causing slowdown of decoding.
As $d\times d$ surface code requires at least $d$ rounds of syndrome measurements, average throughput of decoding must be $O(d)$ or faster to avoid an exponential backlog.


% As each measurement of an ancilla qubit is a binary value the syndrome $S$ can be mathematically represented as a binary tensor. 
% As decoding of X-errors (from the data from Z ancillas) and Z-errors (from the data from X ancillas) occur independently they can be represented as separate tensors.
% Thus the syndrome $S$ is represented as two binary tensors of $T\times d\times(d-1)$ each where each element is "1" if it corresponds to a non-trivial measurement and $T$ is the number of rounds of measurement which should be at least $d$.
% The two binary tensors are called X-syndrome and Z-syndrome in CSS surface code. 
% As the decoding process for both syndromes is similar for the rest of the paper the difference between the two tensors are ignored and explained for one syndrome.
% % Figure \todo{fig} shows a visualization of an X-syndrome.



The fastest and most accurate way to decode is using a lookup table (LUT) decoder. 
However, as a surface code of distance $d$ requires $2^{T\times d \times (d-1)}$ entries, a LUT is not scalable and is only feasible for very small surface codes. 
Thus approximation algorithms such as Minimum Weight Perfect Matching (MWPM) and Union Find (UF) are necessary for scalable QEC. 


\subsubsection{Minimum Weight Perfect Matching}
Minimum Weight Perfect Matching (MWPM) reconstructs the syndrome as a fully connected graph where each vertex is a non-trivial measurement in the syndrome and each edge is the most-likely error chain resulting in the two non-trivial measurements.
Each edge is weighted based on the probability of the respective error chain occurring. 
For this step the negative of the logarithm of the probability of the error chain occurring is used as then error chains with highest probability will have the lowest value.
An MWPM algorithm then selects a perfect matching of the graph with lowest weight. 
Such a perfect matching corresponds to an error pattern with the highest probability based on the mapping of the syndrome to the graph. 
%It should be noted that MWPM does not find the error pattern with the highest probability as mapping the syndrome to a fully-connected graph ignores information related to error patterns with more than two non-trivial measurement values.
The computational complexity of MWPM depends on the algorithm used for MWPM. 
Blossom V ~\cite{kolmogorov2009blossom} is one of the most efficient MWPM algorithms with a worst-case time complexity of $O(d^9)$.    
\end{comment}




==> app_serialUF.tex <==

\pargaraph{Union-Find (UF) Decoder} is a fast surface code decoder design first suggested by Delfosse and Nickerson~\cite{delfosse2017almost}. 
According to~\cite{yue2021interpretation}, it can be viewed as an approximation to the blossom algorithm that solves MWPM problems.
It has a worst case time complexity of $O(d^3\alpha (d))$, where $\alpha$ is the inverse of Ackermann’s function, a slow growing function that is less than three for any practical code distances. 
\lin{Please give the average since that is what used later.}

\algref{alg:serialuf} describes the UF decoder.
% For clarity, we will only use X errors below as Z errors can be independently dealt with in the same way. Furthermore \autoref{fig:uf_example} visualizes a two dimensional decoding graph for convenience and omits measurement errors. 
In the UF decoder, each edge $e\in \mathbf{E}$ has a weight and a growth, denoted by $e.w$ and $e.g$, respectively. $e.g$ is initialized with $0$ and the decoder may grow $e.g$ until it reaches $e.w$. When that happens, we say the edge is \emph{fully grown}.


The decoder maintains a set of odd clusters, denoted by $\mathcal{L}$. $\mathcal{L}$ is initialized to include all $\{v\}$ that $v\in\mathbf{V}$ is non-trivial (\lineref{line:initial_list}. 
 Each cluster $C$ keeps track of whether its cardinality is odd or even as well as its root element.

The UF decoder iterates over growing and merging the odd cluster list until there are no more odd clusters (inside the \textbf{while} loop of \algref{alg:serialuf}). 
Each iteration has two stages: Growing and Merging. 
In the \emph{Growing} stage, each odd cluster ``grows'' by increasing the \emph{growth} of the edges incidental to its boundary. 
This process creates a set of \emph{fully grown} edges $\mathcal{F}$ (\lineref{line:grow-start} to \lineref{line:grow-end}). 
The Growing stage is the more time-consuming step as it requires traversing all the edges in the boundary of all the odd clusters and updating the global edge table. 
Since the number of edges is $O(d^3)$, the sequential find UF decoder is not scalable for surface codes with large $d$. 

In the \emph{Merging} stage, the decoder goes through each fully-grown edge to merge the two clusters connected by the edge. 
When two clusters merge, the new cluster may become even. 

When there is no more odd cluster, the decoder finds a correction within each cluster and combines them to produce the correction pattern (\lineref{line:peeling}). 
% We do not provide further details because this step runs only once and does not have a significant impact on worst case time complexity.


%\yue{not necessarily true, peeling algorithm requires iterating over all grown edges to build spanning tree; maybe just skip peeling algorithm, replace it with ``build correction within each cluster''. It can be either a peeling algorithm or a random selected matching, or the parallel implementation of correction building. Any of these work fine because they don't differ by logical error.}
% We next describe the GROW  (\lineref{line:grow}), TOUCH and MERGE (\lineref{line:merge})functions (\lineref{line:touch}) shown in \autoref{alg:serialuf}. 
% GROW$(C_i)$, increases \emph{growth\_value} of each edge ($e_{ij}$) crossing the cluster boundary $C_i$ ($e_{ij} = \{v_i,v_j | v_i \in C_i~\&~ v_j \notin C_i\}$) by 1 unit. 
% Parameter \emph{growth\_value} which is between 0 and weight of the edge, is an indication of how far the cluster has grown across each edge in its boundary. 
% When the \emph{growth\_value} is equal to the weight of the edge, the edge is labeled as \emph{fully\_grown} and the vertex at the other end of the edge is added to the cluster.
% TOUCH$(C_i, C_j)$ returns true when two clusters touch each other. 
% This occurs when either the sum of growth values of an edge between the two clusters ($e_{ij} = \{v_i,v_j | v_i \in C_i~\&~ v_j \in C_j\}$) is equal to the weight of the edge or when two clusters share a vertex. 
% When two clusters touch each other they are merged into a single cluster by MERGE $(C_i, C_j)$. 
% MERGE $(C_i, C_j)$ creates a new cluster with a boundary which includes all the vertices in $C_i$ and $C_j$. 
% Each edge in the new cluster has a \emph{growth\_value} equal to the sum of \emph{growth\_value}s for that edge (if included) in $C_i$ and $C_j$. 


% The algorithm begins with clustering each non-trivial measurement into an individual cluster, which is always a set of odd clusters (\lineref{line:initial_list}). 
% The algorithm continues until all clusters become even clusters. 
% Since a cluster touching the boundary indicates that cluster contains an error chain connected to the boundary and based on the parity of such clusters the presence of X (or Z) errors in the surface code can be identified  (\lineref{line:peel_start} to \lineref{line:peel_end}). 
% Authors of \cite{yue2021interpretation} shows the internal similarities between the Blossom algorithm used for MWPM and UF.




% \begin{figure*} [!ht]
%     % \renewcommand*\thesubfigure{(\alph{subfigure})}  % add parentheses manually
% 	\centering
% % 	\includegraphics[width=0.80\linewidth]{figures/syndromes.pdf}
%     \begin{subfigure}{0.17\textwidth}
% 	    \centering
%         \includegraphics[width=1\textwidth]{figures/uf_1.png}
%         \caption{}
%         \label{fig:uf_1}
%     \end{subfigure}
%     %\hfill
%     \begin{subfigure}{.17\textwidth}
% 	    \centering
%         \includegraphics[width=1\textwidth]{figures/uf_2.png}
%         \caption{}
%         \label{fig:uf_2}
%     \end{subfigure}
%     \begin{subfigure}{.17\textwidth}
% 	    \centering
%         \includegraphics[width=1\textwidth]{figures/uf_3.png}
%         \caption{}
%         \label{fig:uf_3}
%     \end{subfigure}
%     \begin{subfigure}{.17\textwidth}
% 	    \centering
%         \includegraphics[width=1\textwidth]{figures/uf_4.png}
%         \caption{}
%         \label{fig:uf_4}
%     \end{subfigure}
%     \begin{subfigure}{.17\textwidth}
% 	    \centering
%         \includegraphics[width=1\textwidth]{figures/uf_5.png}
%         \caption{}
%         \label{fig:uf_5}
%     \end{subfigure}
% 	\caption{Stages of the union-find decoder visualized on the decoding graph. 
% 	Each vertex corresponds to a measurement value and non-trivial measurement values are shown in red. Odd clusters are shown in orange and even clusters are shown in green. Each edge has a weight of 2. (a) Initially each non-trivial measurement value is assigned to a separate cluster. (b) All odd-clusters grow along the edges. (c) $C_1$ and $C_2$ touch each other hence merged together to form new even cluster $C_5$ (d) Odd clusters, $C_3$ and $C_4$ keep growing (e) $C_3$ and $C_4$ merge together. Clustering finishes at this stage as there are no remaining odd clusters. It should be noted that the actual decoding graph is a 3-D graph and not a 2-D graph due to multiple measurement rounds.
% 	}
% 	\label{fig:uf_example}
% \end{figure*}

% As both sequential MWPM~\cite{fowler2014minimum} and sequential UF~\cite{delfosse2017almost} both have complexities significantly higher than $O(d)$  parallel implementations are necessary to avoid exponential slowdown of decoding.


\begin{algorithm} [!t]
\DontPrintSemicolon
% \SetAlgoNoLine
\caption{Union Find Decoder (Integer Weighted)}\label{alg:serialuf}
\footnotesize
\setcounter{AlgoLine}{86}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{A decoding graph $\mathcal{G}(\mathbf{V}, \mathbf{E})$ with X (or Z) syndrome}
\Output{A correction pattern}
\% Initialization\\
% \ForEach{$e \in \mathbf{E}$}{
%     $e.growth\gets 0$\label{line:set_edges}
% }
    \ForEach{$v\in \mathbf{V}$}{
        \If{$v$ is non-trivial}{
            Create a cluster $\{v\}$
        }
        \label{line:initial_list}
    }

\While{there is an odd cluster}{ \label{line:loop_start}
    \% Growing\\
    $\mathcal{F}\gets \emptyset$\\
    \ForEach{odd cluster $C$}{
    \label{line:grow-start}
         \ForEach{$e=<u,v>$, $u\in C, v\not\in C$ }{
        % \ForEach{$e=<u,v> \in C.B$ }{
            \If{$e.growth < e.w$}{ %If not fully grown
                $e.growth\gets e.growth+1$ \label{line:grow_serial}\\
                \If{$e.growth = e.w$}{ %If not fully grown{
                    $\mathcal{F} \gets \mathcal{F} \cup \{e\}$ \label{line:fusion_set}
                }
            }
        }
        
    }\label{line:grow-end}
    \% Merging\\
    \ForEach{$e = <u,v> \in \mathcal{F}$}{
        UNION($u$, $v$) \label{line:merge}

    }
}
\label{line:loop_end}
\textup{Build correction within each cluster} \label{line:peeling}
\end{algorithm}
